How does the preparation strategy influence the gold cap of thermophoretic Janus swimmers and their propulsion?

The motion of partly gold (Au)-coated Janus particles under laser irradiation is caused by self-thermophoresis. Despite numerous studies addressing this topic, the impact of the preparation method and the degree of coverage of the particle with Au on the resulting thermophoretic velocity has not yet been fully understood. A detailed understanding of the most important tuning parameters during the preparation process is crucial to design Janus particles that are optimized in Au coverage to receive a high thermophoretic velocity. In this study, we explore the influence of the fabrication process, which changes the Au cap size, on the resulting self-propulsion behavior of partly Au-coated polystyrene particles (Au-PS). Additionally, also the impact of an underlying adhesion chromium layer is investigated. In addition to the most commonly used qualitative SEM and EDX measurements, we propose a novel technique utilizing AFM studies to quantify the cap size. This non-invasive technique can be used to determine both the size and the maximum thickness of the Au cap. The Au cap size was systematically varied in a range between about 36 % and 74 % by different preparation strategies. Nevertheless, we showed that the differing Au cap size of the Janus particles in this range has no effect on the thermophoretic velocity. This surprising result is discussed in the paper.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
